Teaching Algorithmic Reasoning via In-context Learning

Large language models (LLMs) have shown increasing in-context learning capabilities through scaling up model and data size. Despite this progress, LLMs are still unable to solve algorithmic reasoning problems. While providing a rationale with the final answer has led to further improvements in multi-step reasoning problems, Anil et al. 2022 showed that even simple algorithmic reasoning tasks such as parity are far from solved. In this work, we identify and study four key stages for successfully teaching algorithmic reasoning to LLMs: (1) formulating algorithms as skills, (2) teaching multiple skills simultaneously (skill accumulation), (3) teaching how to combine skills (skill composition) and (4) teaching how to use skills as tools. We show that it is possible to teach algorithmic reasoning to LLMs via in-context learning, which we refer to as algorithmic prompting. We evaluate our approach on a variety of arithmetic and quantitative reasoning tasks, and demonstrate significant boosts in performance over existing prompting techniques. In particular, for long parity, addition, multiplication and subtraction, we achieve an error reduction of approximately 10x, 9x, 5x and 2x respectively compared to the best available baselines.

==> commented_stuff.tex <==
%(related experimental results for this would be various gsm8k exps)

%Humans learn through curriculum learning to master increasingly complex skill sets. The idea of curriculum learning has been explored in deep learning, but usually in the context of ordering the examples by difficulty in gradient-based learning, or reducing the problem into sequential solution steps (e.g. least-to-most prompting). With the emergence of in-context learning capabilities, a new type of curriculum learning can be unlocked, which is a more systematic mastery of complex algorithms or thinking patterns through building on top of simpler subroutines. 

%    --- 




%The first step toward continuous skill acquisition through prompting is to improve the model’s ability to learn skills through in-context learning. We want to study how various forms of prompt impact algorithmic learning.


%    --- Humans don't just learn from seeing examples, especially for more complex tasks, but rather learn the underlying process of solving the task, which allows us to understand how to solve the task in new settings. Similarly, if the model learns an algorithm for solving a problem, we would get OODG for free.
    

% In this work we focus on investigating

%In order to extend the use of current LLMs to solve complex tasks, The ability of models to reason given the provided information and go beyond pattern matchning has been of interest Despite these progress, LLMs are still unable to solve algorithmic reasoning problems, which require the model to learn an algorithm for a given task.
%mention few-shot prompting (also called in-context learning)  Introduce OODG (in particular systematic generalization, e.g. length generalization) as a general test bed to see if models are actually learning to reason using the underlying rules or algorithm that govern a task/dataset.


 
% - Why in-context learning (particularly in the context of reasoning and algorithmic reasoning)?

%  Due to the observed superior performance of in-context learning to gradient-based learning, we focus on in-context learning.  the capabilities of language models to learn algorithmic reasoning through in-context learning.
%     --- Better results when learning from few shot and instructions (cite length generalization paper, maybe others)
    
%     --- Learn / leverage more general features
    
%     --- Finetuning leads to overfitting or exploiting of correlational features (cite length gen~\cite{anil2022exploring}, maybe others).
    
% - Rationale-enabled prompting also exhibits better scaling properties.

%- Introduce algorithmic reasoning as a subset of this topic (what is the difference between algorithmic reasoning and symbolic reasoning (or other types of reasoning)?


    


% Large language models have been shown to exhibit many emergent capabilities such as XXX. One of the most exciting capabilities is in-context learning, which is the ability to instruct the model in some way through prompting. In-context learning presents a powerful alternative to gradient-based learning. It allows us to modify the model's behavior without making changes to the underlying weights. Thus we do not risk unforeseen adverse changes to the model as a result of finetuning, etc. The other benefit is that in-context learning is more sample efficient, often requiring only a few examples to learn a task.

%- Underexplored continual learning / curriculum learning through in-context. Why is this desirable?





% If we think of rationales as roughly providing a guidance for how to think about the problem, the question arises on how precisely we can specify such a thinking pattern and how well we can control the model's behavior.
